Automated Smell Detection and Recommendation in Natural Language Requirements

Requirement specifications are typically written in natural language (NL) due to its usability across multiple domains and understandability by all stakeholders. However, unstructured NL is prone to quality problems (e.g., ambiguity) when writing requirements, which can result in project failures. To address this issue, we present a tool, named Paska, that takes as input any NL requirements, automatically detects quality problems as smells in the requirements, and offers recommendations to improve their quality. Our approach relies on natural language processing (NLP) techniques and a state-of-the-art controlled natural language (CNL) for requirements (Rimay), to detect smells and suggest recommendations using patterns defined in Rimay to improve requirement quality. We evaluated Paska through an industrial case study in the financial domain involving 13 systems and 2725 annotated requirements. The results show that our tool is accurate in detecting smells (89% precision and recall) and suggesting appropriate Rimay pattern recommendations (96% precision and 94% recall).

==> RequirementOverallGrammar.tex <==
REQUIREMENT: SCOPE? CONDITION_STRUCTURES? ARTICLE? ACTOR MODAL_VERB not?  SYSTEM_RESPONSE.
SCOPE: For MODIFIER? TEXT (and MODIFIER? TEXT)?,
CONDITION_STRUCTURE: WHILE_STRUCTURE|WHEN_STRUCTURE|WHERE_STRUCTURE|IF_STRUCTURE|TEMPORAL_STRUCTURE
WHILE_STRUCTURE: While PRECONDITION_STRUCTURE
WHEN_STRUCTURE: When TRIGGER
WHERE_STRUCTURE: Where TEXT
IF_STRUCTURE: If PRECONDITION_STRUCTURE|TRIGGER
TEMPORAL_STRUCTURE:  (Before|After|Every) TEXT
CONDITION_STRUCTURES: CONDITION_STRUCTURE ( (,|and|or|,or|,and) CONDITION_STRUCTURE)*, then?

==> bio.tex <==
\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}

==> revision_1/metareview.tex <==
\noindent\textbf{Editor} \\

\noindent Thanks for your submission to the IEEE Transactions on Software Engineering. While there are different opinions among the reviewers, there is a consensus that the paper tackles an important topic and has the potential to make an interesting contribution.
\hfill \break

%\vspace{-0.5em}
\noindent However, some of the reviewers have some major concerns about the soundness and novelty of the work that require a better framing of the solution and additional clarifications.
In particular, the reviewers have highlighted the following three issues:

%\vspace{-0.5em}
\metarwcomment{m1}{
- (novelty of the) contribution: Since the paper stems from a previous contribution, the authors should clearly state the novelty of the current work with respect to the previous one. In addition, the contribution has not been precisely described: the authors say that  Paska provides RE authors with guidance on resolving quality defects, but this is limited to suggesting Rimay patterns (and these are not shown to be comparable).
}

%\vspace{-0.5em}
\response{
Previous work~\cite{VeizagaATSB21} defines and validates the Rimay language while this work detects requirement smells and proposes recommendations to rectify them based on the concepts in Rimay.
In response to comment~\refcomment{r1c1}, we have improved the writing in Section~\ref{sec:intro} to clearly describe our contributions.
}

%\vspace{-0.5em}
\response{
Regarding the comment on Rimay patterns, these are structured recommendations and align with the best practices for writing functional requirements in Rimay, which enforces the following quality attributes: completeness, clarity, correctness, and atomicity.
Hence, suggesting Rimay patterns as recommendations helps analysts improve the quality of their requirements by clearly indicating which requirement segment is missing, needs to be re-ordered, or changed.
Our response to comment~\refcomment{r2c2} further clarifies this and provides a concrete example that illustrates how an analyst applies the suggested Rimay pattern to address smells in a natural language (NL) requirement.
}

%\vspace{-0.5em}
\response{
Comment~\refcomment{r2c3} concerns about whether \TOOL is a promising solution and compares it with a hypothetical RE chatbot.
Firstly, our experiment results factually indicate that \TOOL is indeed promising, based on the largest set of industrial requirements to date in any study.
Additionally, we note that drawing a direct comparison between our tangible tool, carefully evaluated in an industrial context, and a hypothetical RE chatbot system cannot lead to a reliable conclusion. ChatGPT-like technologies may not be well-suited for incorporating newly introduced research outcomes, such as Rimay, particularly in situations where substantial training data is lacking, such as requirements written in Rimay. This will have to be investigated by additional research in the future, not in this already large paper.
For further details, please refer to our response to the comment.
}

%\vspace{-0.5em}
\metarwcomment{m2}{
\noindent - Lack of details and relevant information; in particular, the paper should include the process used to derive the quality attributes to consider from Rimay and a clear link between these attributes and others used in the literature. Also, the explanation of the procedure for identifying smells and reaching saturation is not sufficiently detailed.
}

%\vspace{-0.5em}
\response{
Regarding the comment on the derivation process for the quality attributes, we admit that our writing in Section~\ref{subsec:smells} was misleading.
\TOOL detects requirement smells that violate the following quality attributes: completeness, clarity, atomicity, and correctness, which are enforced by Rimay.
Note that these quality attributes were considered when evaluating Rimay with practitioners in a prior study~\cite{VeizagaATSB21}.
Our response to comment~\refcomment{r1c2} describes our revision in detail to clarify that Rimay enforces these quality attributes when writing requirements.
}

%\vspace{-0.5em}
\response{
In response to the comment on a clear link between our quality attributes and others proposed in the literature,
we note that the quality attributes enforced by Rimay, particularly completeness and clarity, align with those prominently studied in the literature~\cite{MontgomeryFBSM22}, indicating they correspond to commonly observed quality issues in requirements engineering.
Regarding the atomicity of a Rimay requirement, it contributes to improving the other quality attributes, such as clarity and verifiability.
However, the correctness of a Rimay requirement, in this article, is different from the notion of correctness in existing works~\cite{Denger2005}, which concerns whether a requirement accurately captures users' needs.
In our context, the correctness of a Rimay requirement pertains to the correct arrangements of words and phrases defined in the Rimay rules.
We have provided a more detailed explanation about this concern in our response to comment~\refcomment{r1c2}.
}

%\vspace{-0.5em}
\response{
Regarding the comment on the procedure for identifying smells and reaching saturation, we have provided the requested details, including the researchers' backgrounds, the inspection process, and threats to validity, in our response to comment~\refcomment{r1c3}.
}

\vspace{3em}
\metarwcomment{m3}{
\noindent - Additional expected contribution: since the paper proposes a tool for a company, the readers might expect an evaluation with users to understand whether the tool is helpful and get convinced that the solution is considered useful by the company.
}

%\vspace{-0.5em}
\response{
As written in our responses to comments~\refcomment{r1c9} and \refcomment{r3c16}, \TOOL is an automated smell detection and recommendation tool that does not require user intervention.
Therefore, when evaluating \TOOL, we did not conduct user-centric evaluations.
Such evaluations are typically required for tools that rely on user input or interactions to operate in an optimal and accurate manner.
Hence, we believe the absence of user studies does not undermine the validity of our findings.
Nevertheless, we acknowledge the importance and value of user studies in technology evaluation, especially in terms of the economic benefits from the users' perspective. However, this cannot be yet an additional part to this already large paper. 
To clarify this further, we have enhanced our discussion on this research direction in Section~\ref{sec:qa_conclusions}.
}

\clearpage

==> smells_rimaypatterns.tex <==
\section{Requirements Smells and Rimay Patterns}
\subsubsection{Software Requirement Specifications}
\label{qa:sub2secSRS}
One of the inputs in our approach is software requirements specifications.
These specifications contain a set of NL requirements.
In our context, SRSs are written in English using MS Word document format.
We collected SRSs from our industrial partner Clearstream. The financial analysts provided us with a set of two SRSs acknowledging that the SRSs contain an early version of NL requirements and that further iterations of revisions were expected. The SRSs contain 384 requirements and were written by different business analysts at Clearstream. Each SRS contains a different number of requirements.
These SRSs describe different types of project, including updates to existing applications, compliance of the application with new regulations, creation of new applications, and description of the migration of existing applications to new platforms.  
%The SRSs were provided to us on an opportunistic manner.

%For the creation of our approach, we used two SRSs that contain 384 requirement. %The remaining SRSs were used for the evaluation of our approach. 

%Clearstream typically has to deal with SRSs written in NL that are created by domain experts (from now on, we refer to them as \financial analysts")
%who do not necessarily possess sufficient expertise in requirements elicitation and definition.
%Rimay language was developed after analyzing the information content of a large set of requirements from the financial domain. Furthermore, the initial validation of Rimay was conducted in company from the financial domain.
%Recall from Section~\ref{sec:qa_background} that Rimay provides constructs and by design the requirements produced by Rimay are complete, unambiguos, and testeable.
\subsubsection{Requirements Smells}
\label{subsec:qa_smells}

This section aims to answer RQ1. To do so, we propose a set of 10 smells that reflect the most common semantic and syntactic errors found in the NL requirements.

The smells were borne out of an analysis of NL requirements that violate the quality features that the Rimay language enforces in their constructs and concepts. 
We use Rimay  because: (1) there is a match between the domain where Rimay is applicable and our case study context, and (2) the Rimay concepts and constructs are characterized by providing precise syntax and semantics for defining functional requirements. 

To derive the quality features enforced by Rimay constructs, we analyze concepts and constructs that are part of the syntax and semantics of Rimay. We distinguish the following quality features for which the requirements written in Rimay should account for:
%in the syntax and semantics  characteristics
\begin{enumerate}
    \item Completeness refers to the presence of all the information content of the requirement to give a complete and precise idea.
    \item Clearness refers to the usage of structures, phrases, and words that are free of ambiguity.
    \item Atomic requirements refer to a natural language statement that describes a single system function.% usage of the best practices recommended in the field of requirements engineering.
    \item Correctness refers to enforcing the presence of correct information content in the correct order of appearance.
\end{enumerate}

%as a baseline of the good syntactic and semantic quality features that the requirements should account for
%Recall from Section~\ref{sec:qa_background} that Rimay is a CNL for writing requirements in the domain of information systems, initially validated in the financial domain.

%Rimay has rules to define scope, condition, and system response.

To derive the smells, we analyzed a set of 384 NL requirements provided by our industrial partner to find requirement smells that violate the quality features of completeness, clearness, atomic requirements, and correctness.
Table~\ref{table:reqSmells} shows the ten smells we identified. The first column shows the name of the smell. The second column shows the description of the smell. The third column indicates the quality characteristic that the smell violates. Finally, the fourth column indicates the extent to which the smell affects. More specifically,  the part of the requirement in which the smell affects or if the smell affects the whole requirement. We use two types of extent: requirement and segment. 
The proposed smells were validated by our industrial partner who agreed that the list includes errors that are frequently performed by business analysts when writing NL requirements. 




\begin{table}[]
\caption{Requirements smells}
\label{table:reqSmells}
\begin{tabular}{p{2.8cm} | p{7cm}| p{1.7 cm}|l}
\textbf{Smell Name} & \textbf{Description} & \textbf{Quality characteristics} &  \textbf{Extent}\\
\hline

Non-atomic & Non-atomic happens when there is more than one action in the system response & Atomic requirement & \multirow{5}{*}{Requirement}\\
\cline{1-3}
Incomplete requirement & Incomplete requirement happens when the requirement does not have a system response but has other optional parts, i.e., condition and  scope & Completeness & \\
\cline{1-3}
Incorrect order requirement &  Incorrect order occurs when  a condition is located after the system response. This construct leads to a vague interpretation of the occurrence of the condition & Correctness  \\
%It is not clear when the condition will take place.  After the system response, before or at the same time of the system response. & Correctness & \\
\cline{1-3}
Coordination ambiguity & Coordination ambiguity happens when a requirement has two or more conditions and these conditions are connected either by: (a) a coordinated conjunction "or", (b)comma, or (c) nothing  & Clearness & \\
\cline{1-3}
Not a requirement & Not a requirement happens when the requirement does not contain any part, i.e.,  scope, condition, and system response.  & Correctness & \\
\hline
Incomplete condition & Incomplete condition happens when the condition lacks of either actor or verb  & Completeness & \multirow{5}{*}{Segment}\\
\cline{1-3}
Incomplete system response & Incomplete system response happens when the system response lacks of either the actor, the modal or the verb. & Completeness &  \\
\cline{1-3}
Incomplete scope & Incomplete scope happens when the scope misses a noun. 
%The scope phrase is composed by the preposition "for" and a noun phrase. This smell occurs when the Scope does not have any noun phrase after the preposition "for". 
& Completeness & \\
\cline{1-3}
Passive voice & Passive voice happens when either the condition or system response are described in the passive voice and the description misses the subject.  
%the grammatical construction is present in the requirementused when we  want to emphasize the action and the object of a sentence rather than subject. When this structure is used is easy for the business analyst to omit the actor of a requirement unless the by-phrase is used. In our context this smells occurs when there is the passive construct and it is not mention the subject. The passive voice smells occurs in the condition or in the system response.
& Completeness &  \\ 
\cline{1-3}
Not Precise Verbs & Not precise verb happens when either the verb of the condition or system response is not precise enough. The verb misses a precise action.  The list of our not precise verbs include: "accomplish", "account",  come, consider, default, define, do, get, make, perform, "process", propose, make, raise, "read", set, "support", "want". This list was curated by the business analysts from Clearstream & Clearness &  \\
\end{tabular}
\end{table}

\textbf{Answer to RQ1: } First we identify the quality characteristics enforced by Rimay which are: atomic requirements, completeness, correctness, and completeness. Second, on a set of 381 requirements, we identified ten requirements smells that violate the aforementioned quality characteristics. We derived 10 smells. Our industrial partner confirmed that our list of requirements smells reflect the common problems that business analysts made while specifying NL requirements.


% \begin{table}[]
% \caption{Requirements smells}
% \label{table:smellExtent}
% \begin{tabular}{l|p{7.5cm}}
% \textbf{Extent} & \textbf{Smells} \\
% \hline
% Requirement & Incomplete requirement, incorrect order requirement, not a requirement, coordination ambiguity, non-atomic requirement\\
% \hline
% Segment & incomplete condition, incomplete system response, incomplete scope, passive voice, and  lexical ambiguity \\
% \end{tabular}
% \end{table}


%One of the author analyzed natural language requirements to identify problems that make the requirement not understandable. The idea is to extract requirements smells and build a catalogue.

% The smells that concern to the scope requirement are: (1) non-atomic requirement, (2) incomplete requirement, (3) incorrect order requirement, (4) coordination ambiguity, and (5) not requirement. 


% The smells that concern to the segment scope are: (1) incomplete condition, (2) incomplete system response, (3) incomplete scope, (4) passive voice, and (5) lexical ambiguity. 




\subsubsection{Rimay Patterns}
\label{subsec:rimay_patterns}
%What is it ? Why do you need ? How did you convey? The results 
%RQ3: How can we suggest requirements templates to improve the quality of requirements?
In this section, we present the list of ten requirements patterns derived from the concepts and constructs of the Rimay language. These patterns will be used by our approach to provide suggestions to the business analysts when our approach detects smell(s) in NL requirements. If analysts follow our suggestions and rewrite the requirements using the suggested patterns, the requirements will be free of smell(s) and  will contain the quality characteristics enforced by Rimay, i.e., completeness, clearness, atomic requirements, and correctness.
To derive the requirements patterns, we create a conceptual model for the concepts pertinent to the Rimay language. Figure~\ref{fig:rimayConceptualModel} shows a high level of abstraction of the Rimay concepts. The model defines five concepts for the Requirement, five concepts for the Condition\_Structure, and 58 concepts for the Action\_Phrase (Figure~\ref{fig:rimayConceptualModel} only shows a few concepts for Action\_Phrase). Furthermore, the model defines the concept Condition shared by the concepts While\_Structure, If\_Structure, and Temporal\_Structure. The concept Trigger is shared by the concepts If\_Structure, When\_Structure, and Temporal\_Structure. The concept Free\_Expression is shared by the concepts When\_Structure, Where\_Structure and Temporal\_Structural. The concept Time\_Adverb belongs to the Temporal\_Structure.

We analyze the possible combinations of the aforementioned concepts to create requirement patterns. The requirement patterns contain valid sequences of Rimay concepts. 

% The purpose of suggesting requirement pattern is to provide a starting reference for the usert to convert the requirement into the Rimay language.
% The proposed requirement patterns aim at providing structures with different combinations of the concepts and  constructs 
% Using the conceptual model of Rimay we derive patterns from Rimay. 
%On the contrary, having a low level of abstraction of the Rimay concepts will requirement patterns that provide very specific concepts could lead as to have hundreds of requirement patterns.  
%idea is to have general concepts rather than specific ones. 
%Figure~\ref{fig:rimayConceptualModel} does not include all the Rimay concepts  because we aim to propose requirement patterns that contain the are the starting guide to write the requirement in Rimay. 


\begin{figure}[htpb]
\centering
 \centerline{\includegraphics[width=\linewidth]{ConceptualModel.pdf}}
\caption{Rimay conceptual model}
\label{fig:rimayConceptualModel}
\end{figure}
%analyzed during the derivation of the requirements smells.
Table~\ref{fig:rimayPatterns} outlines the ten requirement patterns derived from the conceptual model of the Rimay language. The first column shows the name of the pattern. The second column shows the pattern. Finally, the third column depicts an example of the applicability of the pattern.
Table~\ref{fig:rimayPatterns} does not include all the keywords from Rimay concepts and also does not include the templates for the Action-Phrases. Refer to our previous work~\cite{DBLP:journals/ese/VeizagaATSB21} for a complete reference to the concepts and constructs of the Rimay language. 

The proposed patterns aim at providing a point of reference of the sequence of Rimay concepts. We assume that the analysts have a previous knowledge of the concepts and constructs of Rimay language. Recall from Section~\ref{sec:qa_background} that the Rimay editor provides useful features that help analysts to write the requirements. 
  
%Once the user will start writing the requirement int he editionwill help  shows  general template that the analyst has to use depending on the action phrase. 

 %The complete list of action phrases and more information are available in. For all the types of ACTION PHRASE rules are available in The Rimay patterns are shows concepts at high level of abstraction.
% The idea is that the Rimay is a language where the user needs to know in advance the structure to Rimay is a language that  does not provide any pattern.







%Once our tool identifies smells on NL requirements. Our tool identifies the syntax  of the requirement and provide a template to the business analysts.  These patterns are going to be used as suggestions for the analysts how they can rephrase NL requirements and writing a requirements free of smells.


 



\begin{table}[htpb]
\centering
 \centerline{\includegraphics[width=1\linewidth]{patterns.pdf}}
\caption{Rimay Patterns}
\label{fig:rimayPatterns}
\end{table}

%We extract patterns from Rimay to produce complete requirements.

% \begin{figure}[htpb]
% \centering
%  \centerline{\includegraphics[width=0.5\linewidth]{ConceptualModel.pdf}}
% \caption{Rimay Conceptual Model}
% \label{fig:approachOverview}
% \end{figure}

%These pattern are going to be used as suggestions for the business analysts when they want to fix the smells tha. The aim is to provide the starting point so that the business analyst can take the template and start to write a requirement.  



 

%Rimay is a language that has  a restricted vocabulary and syntax. Rimay was built after analyzing the syntax of a large set of NL requirements from the financial domain.  %Rimay

%Recall from Section~\ref{sec:qa_background} that a Rimay allows analyst to produce requirements. A requirements produced using Rimay is composed of the  following parts: scope, condition, and system response. 
%For the sake of simplicity, in the context of this paper when we refer to system response we are referring to the actor,  modal verb and system response.
%The presence of the scope condition is optional, but the presence of a system response is mandatory in all requirements.
%Figure 



% 
 % tone down The requirements produced by Rimay are complete, unambiguous and precise.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


%enforcing good syntactic and semantics quality characteristics that requirements should account for. Therefore, we used such quality characteristics as a baseline for quality characteristics that NL  requirements should account for. 
%that Rimay enforces by design. Analyze the concepts and constucts enforced in the syntax of requirements. 

%We analyze We distinguish the following quality characteristics that are enforced by the syntax and semantics of Rimay : %completeness, clearness, atomic-requirements, and correctness. unambiguity orincorrectness misplacement is under correctness 

%Misplacement: The order of appearance of the content if the requirement is incorrect.
%Complete: Incomplete condition, SR, Scope, Passive Voice, Incomplete requirement
%Ambiguity Lexical, coordination
%Best practice: Non atomic,  
%Missplacement, Section: Other text that it is not a requirementincorrect order

%Missplaced Segment: The segment is located where it should not be located.
%Incorrectness: The content is incorrect or inconsistent. Not a requirement. not requirement,



%Non-Atomic requirement happens when there is more than one action in the system response requirements. 
%Incomplete requirement happens when the system response is missing in the requirement but other parts of the requirement such as condition or scope are in the requirement.
%Incorrect order requirement happens when the condition is after the system response. This construct leads to a vague interpretation of the connection between the condition and the system response.  It is not clear when the condition will take place.  After the system response, before or at the same time of the system response.
%For example the requirement:  When the user clicks on the checkbox Display on main page, System-A must open the Alert section when the user launches the Application-A. The requirement has contains two conditions  "When the user is on the Utilities Page" and "when the user launches Application" and a system response " . It is not clear the sequence of the event conditions. This construct leads to not precise explanation of the events.

%Coordination ambiguity in our context happens when the requirement has 2 or more conditions and these conditions are separated by either the coordinated conjuction "or", comma, or no separator word or character.  


%Not a requirement happens when the requirement does not contain any scope, condition, and system response. Section~\ref{sec:qa_background} explains the components of each part.

%Incomplete condition happens when the condition does not have actor or verb. 
%Incomplete system response happens when the system response does not have the actor, modal or verb. 
%Incomplete scope happens when the scope phrase does not have any noun. The scope phrase is composed by the preposition "for" and a noun phrase. This smell occurs when the Scope does not have any noun phrase after the preposition "for".

%Passive voice. It is a grammatical construction used when we  want to emphasize the action and the object of a sentence rather than subject. When this structure is used is easy for the business analyst to omit the actor of a requirement unless the by-phrase is used. In our context this smells occurs when there is the passive construct and it is not mention the subject. The passive voice smells occurs in the condition or in the system response.

% Not precise verb happens when the verb of the condition and system response are not precise enough. They do not convey to a precise action that either the actor of the condition or the actor of the  system response should perform that action. We created a list of not precise verb. This list include the verbs: "accomplish", "account",  come, consider, default, define, do, get, make, perform, "process", propose, make, raise, "read", set, "support", "want". The list was curated by the business analysts from Clearstream. They added the verbs process and verb to our initial list. 


%The Rimay language allows analysts to write requirements using different combinations of the parts of requirements. Recall from Section~\ref{sec:qa_background} that a requirement written in Rimay has the following parts: (a) scope, (b) condition, and (c) system response.
%In our context,  a combination of requirement parts means the order in which the requirement-parts appear and the number of times the requirement-parts appear.


 %of the  Rimay language. The Figures depicts a high  level of abstraction of the concepts. 


%To derive the requirements patterns, we analyze the most frequent combinations of the parts of requirements observed on a set of 384 requirements. In our context,  a combination of parts of the requirement  means different combinations based on the order in which the requirement-parts appear and the number of times the requirement-parts appear.  Recall from Section~\ref{sec:qa_background} that  a requirement written in Rimay has the following parts: (a) scope, (b) condition, and (c) system response. 

%The constructs of Rimay allows business analysts to produce requirements using different combinations based on the order in which the requirement-parts appear and the number of times the requirement-parts appear.  


%considering the presence of the concepts, the order of the concepts and the frequency of the concepts.

%Requirements written in Rimay contain combinations of the aforementioned concepts considering the presence of the concepts, the order of the concepts and the frequency of the concepts we derive 10 requirement patterns  These concepts are used to form different combinations to define requirements.


% The Rimay language allows analysts to write requirements using different combinations of concepts and constructs. In our context, a combination means the order in which the concepts appear in the requirement and the number of times the concepts are present in the requirement.
